Deep-6DPose: Recovering 6D Object Pose from a Single RGB Image

Detecting objects and their 6D poses from only RGB images is an important task for many robotic applications. While deep learning methods have made significant progress in visual object detection and segmentation, the object pose estimation task is still challenging. In this paper, we introduce an end-toend deep learning framework, named Deep-6DPose, that jointly detects, segments, and most importantly recovers 6D poses of object instances from a single RGB image. In particular, we extend the recent state-of-the-art instance segmentation network Mask R-CNN with a novel pose estimation branch to directly regress 6D object poses without any post-refinements. Our key technical contribution is the decoupling of pose parameters into translation and rotation so that the rotation can be regressed via a Lie algebra representation. The resulting pose regression loss is differential and unconstrained, making the training tractable. The experiments on two standard pose benchmarking datasets show that our proposed approach compares favorably with the state-of-the-art RGB-based multi-stage pose estimation methods. Importantly, due to the end-to-end architecture, Deep-6DPose is considerably faster than competing multi-stage methods, offers an inference speed of 10 fps that is well suited for robotic applications.

==> architecture.tex <==
%\subsection{Pose R-CNN}
Our base network is derived from the Mask R-CNN~\cite{Mask-RCNN} with the VGG backbone~\cite{SimonyanZ14}. 
\paragraph{Mask R-CNN:} Let us first brief the Mask-RCNN. Mask R-CNN consists of two main component. The first component, called a Region Proposal Network (RPN), proposes candidate object bounding boxes (RoIs). The second component extracts features using RoIAlign layer~\cite{Mask-RCNN} from each candidate box and performs classification, bounding-box regression, and segmentation. %Two those components share same backbone. 
We refer readers to~\cite{Mask-RCNN} details of Mask-RCNN. 

\junk{
Here we present our adaptation from Mask-RCNN with VGG backbone. The input to our network is a RGB image with the size $480 \times 640$. The Region Proposal Network takes the last feature map of VGG (i.e., $conv5\_3$) as input and output RoIs at different sizes and shapes. We use 15 anchors in the RPN (5 scales which are $16 \times 16$, $32\times32$, $64 \times 64$, $128\times128$ and $256 \times 256$ and 3 aspect ratios which are $2:1$, $1:1$, $1:2$). This design allows the network to detect small objects. For each output RoI of RPN, a fixed-size $7\times7$ feature map is pooled from the $conv5\_3$ feature map using the RoIAlign layer. This pooled feature map is used to regress box coordinate, classify, segment, and estimate 6D pose for the object inside the box.
}

\subsection{Pose R-CNN}
Pose-CNN also consist of two main components, with an identical first component (which is RPN) as Mask R-CNN. In the second component, in parallel to predicting the class, box
coordinate, and segment mask, Pose R-CNN also outputs a 6D pose for each RoI.  

\paragraph{Pose representation}

\paragraph{Multi-task loss function}

\paragraph{Network architecture}


==> data.tex <==
\subsection{Training data}

==> inference.tex <==
\subsection{Inference}
